UIBDiffusion: Universal Imperceptible Backdoor Attack for Diffusion Models

Recent studies show that diffusion models (DMs) are vulnerable to backdoor attacks. Existing backdoor attacks impose unconcealed triggers (e.g., a gray box and eyeglasses) that contain evident patterns, rendering remarkable attack effects yet easy detection upon human inspection and defensive algorithms. While it is possible to improve stealthiness by reducing the strength of the backdoor, doing so can significantly compromise its generality and effectiveness. In this paper, we propose UIBDiffusion, the universal imperceptible backdoor attack for diffusion models, which allows us to achieve superior attack and generation performance while evading state-of-the-art defenses. We propose a novel trigger generation approach based on universal adversarial perturbations (UAPs) and reveal that such perturbations, which are initially devised for fooling pre-trained discriminative models, can be adapted as potent imperceptible backdoor triggers for DMs. We evaluate UIBDiffusion on multiple types of DMs with different kinds of samplers across various datasets and targets. Experimental results demonstrate that UIBDiffusion brings three advantages: 1) Universality, the imperceptible trigger is universal (i.e., image and model agnostic) where a single trigger is effective to any images and all diffusion models with different samplers; 2) Utility, it achieves comparable generation quality (e.g., FID) and even better attack success rate (i.e., ASR) at low poison rates compared to the prior works; and 3) Undetectability, UIBDiffusion is plausible to human perception and can bypass Elijah and TERD, the SOTA defenses against backdoors for DMs. We will release our backdoor triggers and code.

==> Table/AddGaussianNoise.tex <==
\begin{table}[htbp]
\vspace{-1.0em}
\centering
\setlength{\tabcolsep}{12pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccccc}
\hline
% \multirow{2}{*}{Model} & \multicolumn{8}{c}{Poison Rate (\%)} \\ \cline{2-9} 
Random Noise           & 1\%    & 2\%   &5\%   & 10\%  & 20\%     \\ \hline
{ASR}          & 99\% & 99\% & 100\% & 100\% & 100\%   \\ 
FID          & 19.48 & 19.52 & 19.80 & 19.37 & 19.49   \\ 
MSE          & 2.36E-3 & 1.13E-3 & 8.03E-4 & 3.02E-4 & 5.30E-4   \\
SSIM          & 0.9865 & 0.9929 & 0.9944 & 0.9969 & 0.9957   \\ \hline
\end{tabular}}
\vspace{-1em}
\caption{Robustness of \frameworkname\space against random noise.}
\label{tab:AddGaussian}
\vspace{-0.5em}
\end{table}

==> Table/DetectionRate.tex <==
\begin{table}[htbp]
\vspace{-1.9em}
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccccccc}
\hline
% \multirow{2}{*}{Model} & \multicolumn{8}{c}{Poison Rate (\%)} \\ \cline{2-9} 
\diagbox{Attacks}{Detection Rate}{Poison Rate}            & 0.05    & 0.10   &0.20   & 0.30  & 0.50   & 0.70   & 0.90   \\ \hline
BadDiffusion        & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\%  \\ 
UIBDiffusion (Ours)          & 0\% & 0\% & 0\% & 0 \%& 0\% & 0\% & 0\% \\ \hline
\end{tabular}}
\vspace{-1em}
\caption{Comparison of detection rates between BadDiffusion and \frameworkname\space against Elija over different poison rates.}
\label{tab:detection}
\vspace{-1em}
\end{table}

==> Table/DifferentEpsilon.tex <==
\begin{table}[htbp]
\centering
\setlength{\tabcolsep}{12pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccccc}
\hline
% \multirow{2}{*}{Model} & \multicolumn{8}{c}{Poison Rate (\%)} \\ \cline{2-9} 
$\epsilon$                  & 0.01   &0.02   & 0.03  & 0.04   & 0.05   \\ \hline
{ASR}           & 91\% & 99\% & 99\% & 99\% & 100\%  \\ 
FID           & 19.57 & 19.64 & 19.55 & 19.62 & 19.64  \\ 
MSE           & 1.19E-2 & 2.04E-3 & 1.17E-3 & 1.30E-3 & 2.04E-3  \\
SSIM           & 0.9356 & 0.9877 & 0.9927 & 0.9920 & 0.9877  \\ \hline
\end{tabular}}
\vspace{-1em}
\caption{Impact of $\epsilon$ (poison rate: 5\%).}%\hl{any conclusion?}}
\label{tab:epsilon}
\vspace{-2em}
\end{table}

==> Table/DifferentTarget.tex <==
\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccc|c}
\hline
Different Targrt & ASR & FID & MSE & SSIM & Generated Backdoor Target Samples\\ \hline
HAT & 100\% & 21.94 & 2.74E-04 & 0.9981 & \includegraphics[width=1.5cm]{Img/new_0.1.png} \\
CAT & 100\% & 19.64 & 6.11E-03 & 0.9766 & \includegraphics[width=1.5cm]{Img/cat_0.1.png} \\ \hline
\end{tabular}
}
\caption{Target Comparison}
\end{table}


==> Table/DifferentTriggerModel.tex <==
\begin{table}[h!]
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{c|cccc}
\hline
Different Model & ASR & FID & MSE & SSIM \\ \hline
VGG & 100\% & 19.57 & 1.74E-03 & 0.9895 \\ 
ResNet & 100\% & 18.96 & 2.26E-03 & 0.9888 \\ \hline
\end{tabular}
}
\caption{Model Comparison}
\end{table}

==> Table/Elijah_MSE_SSIM.tex <==
\begin{table}[htbp]
\setlength{\tabcolsep}{8pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc}
\hline
     & Gray Box & Stop Sign & \frameworkname \space (Ours) \\ \hline
MSE  &          &           117.2&        101.83\\
SSIM &          &           0.0008&        0.0128\\ \hline
\end{tabular}
}
\caption{}
\label{tab:elijah_mse_ssim}
\end{table}

==> Table/Elijah_main.tex <==
\begin{table}[htbp]
\setlength{\tabcolsep}{3pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc}
\hline
              & \multicolumn{3}{c|}{VillanDiffusion*~\cite{chou2024villandiffusion}} & \multicolumn{3}{c}{\frameworkname \space (Ours)} \\ \hline
Model-Dataset & FID      & ASR      & SSIM      & FID       & ASR       & SSIM       \\ \hline
DDPM        &          &          &           &           &           &            \\
%DDPM-A        &          &          &           &           &           &            \\
NCSN       &          &          &           &           &           &            \\
%NCSN-A        &          &          &           &           &           &            \\
LDM        &          &          &           &           &           &            \\ \hline
\end{tabular}
}
\caption{Resilience of VillanDiffusion and \frameworkname \space against Elijah across different diffusion models. ``*'' denotes results replicated from~\cite{an2024elijah}.}
\label{tab:defense_elijah}
\end{table}

==> Table/MainResult2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\setlength{\tabcolsep}{3pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccccccccccc|cccccccccccc}
\hline
                    & \multicolumn{12}{c|}{\begin{tabular}[c]{@{}c@{}}VillanDiffusion~\cite{chou2024villandiffusion}\\ ($\mathcal{T}$: a gray box) \end{tabular}}                                            & \multicolumn{12}{c}{\begin{tabular}[c]{@{}c@{}}\frameworkname \space (Ours)\\ (Imperceptible Trigger)\end{tabular}}                                         \\ \hline
                    & \multicolumn{4}{c|}{FID}                      & \multicolumn{4}{c|}{MSE}                      & \multicolumn{4}{c|}{SSIM} & \multicolumn{4}{c|}{FID}                      & \multicolumn{4}{c|}{MSE}                      & \multicolumn{4}{c}{SSIM} \\ \hline
Model / Poison Rate & 5\% & 10\% & 20\% & \multicolumn{1}{c|}{50\%} & 5\% & 10\% & 20\% & \multicolumn{1}{c|}{50\%} & 5\%  & 10\% & 20\% & 50\% & 5\% & 10\% & 20\% & \multicolumn{1}{c|}{50\%} & 5\% & 10\% & 20\% & \multicolumn{1}{c|}{50\%} & 5\% & 10\% & 20\% & 50\% \\ \hline
DDPM-C              &  20.35   &   19.87   &   20.85   &  \multicolumn{1}{c|}{25.86}     &   6.17E-2  &   2.78E-4   &   4.41E-5   & \multicolumn{1}{c|}{4.94E-6}     &   0.6958   &   0.9987   &  0.9995    &   0.9998   &  19.57   &   24.51   &   20.52   & \multicolumn{1}{c|}{26.51}     &   1.74E-3  &   5.17E-4   &   2.34E-4   &  \multicolumn{1}{c|}{4.28E-6}     &   0.9895  &   0.9961   &    0.9979  &   0.9992   \\
DDPM-A              &     &      &      & \multicolumn{1}{c|}{}     &     &      &      & \multicolumn{1}{c|}{}     &      &      &      &      &     &      &      & \multicolumn{1}{c|}{}     &     &      &      & \multicolumn{1}{c|}{}     &     &      &      &      \\
NCSN-C              &     &      &      & \multicolumn{1}{c|}{}     &     &      &      & \multicolumn{1}{c|}{}     &      &      &      &      &     &      &      & \multicolumn{1}{c|}{}     &     &      &      & \multicolumn{1}{c|}{}     &     &      &      &      \\
NCSN-A              &     &      &      & \multicolumn{1}{c|}{}     &     &      &      & \multicolumn{1}{c|}{}     &      &      &      &      &     &      &      & \multicolumn{1}{c|}{}     &     &      &      & \multicolumn{1}{c|}{}     &     &      &      &      \\
LDM-C               &     &      &      & \multicolumn{1}{c|}{}     &     &      &      & \multicolumn{1}{c|}{}     &      &      &      &      &     &      &      & \multicolumn{1}{c|}{}     &     &      &      & \multicolumn{1}{c|}{}     &     &      &      &      \\ \hline
\end{tabular}
}
\caption{Main Results}
\label{tab:main_result_2}
\end{table*}

==> Table/MinorPoisonRate.tex <==
% \begin{table}[htbp]
% \centering
% \setlength{\tabcolsep}{12pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|cccc}
% \hline
% % \multirow{2}{*}{Model} & \multicolumn{8}{c}{Poison Rate (\%)} \\ \cline{2-9} 
% Poison Rate              & 0.01    & 0.02   &0.03   & 0.05    \\ \hline
% ASR(Ours)          & 41\% & 95\% & 100\% & 100\%   \\ 
% % FID          & 18.92 & 19.30 & 19.33 & 19.77   \\ \hline
% % MSE          & 0.1140 & 6.65E-3 & 1.06E-3 & 5.30E-4 \\
% SSIM(Ours)          & 0.4681 & 0.9643 & 0.9929 & 0.9967  \\ \hline
% ASR(Villan)          & 41\% & 95\% & 100\% & 100\%   \\ 
% SSIM(Villan)          & 0.4681 & 0.9643 & 0.9929 & 0.9967  \\ \hline
% ASR(BadDiff)          & 41\% & 95\% & 100\% & 100\%   \\ 
% SSIM(BadDiff)          & 0.4681 & 0.9643 & 0.9929 & 0.9967  \\ \hline
% \end{tabular}}
% \vspace{-1em}
% \caption{Minor poison rate on \frameworkname\space.}
% \label{tab:minorpoison}
% \vspace{-1em}
% \end{table}

% \begin{table}[htbp]
% \centering
% \setlength{\tabcolsep}{12pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|l|cccc} \hline
% {Method} & {Poison Rate} & {0.01} & {0.02} & {0.03} & {0.05} \\
% \hline
% \multirow{UIBDiffusion(Ours)} & ASR & 41\% & 95\% & 100\% & 100\% \\
%                 & SSIM & 0.4681 & 0.9643 & 0.9929 & 0.9967 \\ \hline
% \multirow{VillanDiffusion} & ASR & 0\% & 0\% & 0\% & 29\% \\
%                   & SSIM & 3.92E-4 & 1.25E-2 & 1.69E-2 & 0.5971 \\ \hline
% \multirow{BadDiffusion} & ASR & 41\% & 95\% & 100\% & 100\% \\
%                    & SSIM & 0.4681 & 0.9643 & 0.9929 & 0.9967 \\ \hline
% % \multicolumn{6}{l}{\textbf{Poison Rate}} \\
% \end{tabular}}
% \vspace{-1em}
% \caption{Minor poison rate on \frameworkname\space.}
% \label{tab:minorpoison}
% \vspace{-1em}
% \end{table}

\begin{table}[htbp]
\vspace{-1em}
\centering
\setlength{\tabcolsep}{10pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cccc}
\hline
{Method} & {Poison Rate} & {0.01} & {0.02} & {0.03} & {0.04} \\
\hline
UIBDiffusion(Ours) & ASR & 41\% & 95\% & 100\% & 100\% \\
                & SSIM & 0.4681 & 0.9643 & 0.9929 & 0.9967 \\
\hline
VillanDiffusion & ASR & 0\% & 0\% & 0\% & 29\% \\
                & SSIM & 3.92E-4 & 1.25E-2 & 1.69E-2 & 0.5971 \\
\hline
BadDiffusion & ASR & 0\% & 0\% & 0\% & 11\% \\
                & SSIM & 6.2245E-3 & 1.4847E-2 & 1.0897E-2 & 0.3669 \\
\hline
\end{tabular}}
\vspace{-1em}
\caption{\frameworkname\space performance with finer-grained of PR.}
\label{tab:minorpoison}
\vspace{-1em}
\end{table}

==> Table/ModelCompare.tex <==
\begin{table}[htbp]
\setlength{\tabcolsep}{1pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|c|c|c|c|}
    \hline
    \textbf{Model} & \textbf{Trigger} & \textbf{PR} & \textbf{FID} & \textbf{MSE} & \textbf{SSIM} \\
    \hline
    \multirow{10}{*}{{BadDiff}} & \multirow{8}{*}{BOX\_14} & 0 & 5.24 & 0.24 & 4.7405 E-5 \\
    & & 0.05 & & & \\
    & & 0.1 & & & \\
    & & 0.2 & & & \\
    & & 0.3 & & & \\
    & & 0.5 & & & \\
    & & 0.7 & & & \\
    & & 0.9 & & & \\
    \cline{2-6}
    & \multirow{8}{*}{UAP\_NOISE} & 0 & 5.51 & 0.24 & 4.7405 E-5 \\
    & & 0.05 & 2.75 & 5.67 E-2 & 0.9664 \\
    & & 0.1 & 2.75 & 5.22 E-2 & 0.9686 \\
    & & 0.2 & 2.91 & 1.34 E-2 & 0.9911 \\
    & & 0.3 & 2.81 & 2.52 E-2 & 0.9839 \\
    & & 0.5 & 2.92 & 6.22 E-3 & 0.9962 \\
    & & 0.7 & 2.89 & 3.11 E-3 & 0.9980 \\
    & & 0.9 & 2.74 & 7.84 E-5 & 0.9995 \\
    \hline
    \multirow{10}{*}{{VillaDiff}} & \multirow{8}{*}{BOX\_14} & 0 & 18.88 & 0.24 & 3.8012 E-3 \\
    & & 0.05 & 20.35 & 6.17E-2 & 0.6958 \\
    & & 0.1 & 19.87 & 2.78E-4 & 0.9987 \\
    & & 0.2 & 20.85 & 4.41E-5 & 0.9995 \\
    & & 0.3 & 22.74 & 1.38E-5 & 0.9997 \\
    & & 0.5 & 25.86 & 4.94E-6 & 0.9998 \\
    & & 0.7 & 32.39 & 3.42E-6 & 0.9998 \\
    & & 0.9 & 47.70 & 2.87E-6 & 0.9999 \\
    \cline{2-6}
    & \multirow{8}{*}{UAP\_NOISE} & 0 & 18.91 & 0.24 & 3.8012 E-3 \\
    & & 0.05 & 19.57 & 1.74 E-3 & 0.9895 \\
    & & 0.1 & 24.51 & 5.17 E-4 & 0.9961 \\
    & & 0.2 & 20.52 & 2.34 E-4 & 0.9979 \\
    & & 0.3 & 22.24 & 3.19 E-5 & 0.9990 \\
    & & 0.5 & 26.51 & 4.28 E-6 & 0.9993 \\
    & & 0.7 & 32.87 & 3.38 E-6 & 0.9991 \\
    & & 0.9 & 48.46 & 2.88 E-6 & 0.9990 \\
    \hline
\end{tabular}
}
\caption{UIBDiff on BadDiff and VillanDiff}
\label{tab:defense}
\end{table}

==> Table/VillanDiffUAP.tex <==
\begin{table}[htbp]
\setlength{\tabcolsep}{1pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|cccccccc|}
    \hline
    Sampler & P.R. Metric & \multicolumn{8}{c|}{Percentage of Trigger} \\
    \hline
    & & 0\% & 5\% & 10\% & 20\% & 30\% & 50\% & 70\% & 90\% \\
    \hline
    \multirow{3}{*}{DDPM} & FID & 18.91 & 19.57 & 24.51 & 20.52 & 22.24 & 26.51 & 32.87 & 48.46 \\
    & MSE & 0.24 & 1.74E-3 & 5.17E-4 & 2.34E-4 & 3.19E-5 & 4.28E-6 & 3.38E-6 & 2.88E-6 \\
    & SSIM & 3.8E-3 & 0.9895 & 0.9961 & 0.9979 & 0.9990 & 0.9993 & 0.9991 & 0.9990 \\
    \hline
    \multirow{3}{*}{DDIM} & FID & \multicolumn{8}{c|}{\texttimes} \\
    & MSE & \multicolumn{8}{c|}{\texttimes} \\
    & SSIM & \multicolumn{8}{c|}{\texttimes} \\
    \hline
    \multirow{3}{*}{DPM Soler 02} & FID & \multicolumn{8}{c|}{\texttimes} \\
    & MSE & \multicolumn{8}{c|}{\texttimes} \\
    & SSIM & \multicolumn{8}{c|}{\texttimes} \\
    \hline
    \multirow{3}{*}{DPM Soler 02++} & FID & \multicolumn{8}{c|}{\texttimes} \\
    & MSE & \multicolumn{8}{c|}{\texttimes} \\
    & SSIM & \multicolumn{8}{c|}{\texttimes} \\
    \hline
    \multirow{3}{*}{DPM Soler 03} & FID & \multicolumn{8}{c|}{\texttimes} \\
    & MSE & \multicolumn{8}{c|}{\texttimes} \\
    & SSIM & \multicolumn{8}{c|}{\texttimes} \\
    \hline
    \multirow{3}{*}{DPM Soler 03++} & FID & \multicolumn{8}{c|}{\texttimes} \\
    & MSE & \multicolumn{8}{c|}{\texttimes} \\
    & SSIM & \multicolumn{8}{c|}{\texttimes} \\
    \hline
    \multirow{3}{*}{DEIS} & FID & \multicolumn{8}{c|}{\texttimes} \\
    & MSE & \multicolumn{8}{c|}{\texttimes} \\
    & SSIM & \multicolumn{8}{c|}{\texttimes} \\
    \hline
    \multirow{3}{*}{HEUN} & FID & \multicolumn{8}{c|}{\texttimes} \\
    & MSE & \multicolumn{8}{c|}{\texttimes} \\
    & SSIM & \multicolumn{8}{c|}{\texttimes} \\
    \hline
    \multirow{3}{*}{LMSD} & FID & \multicolumn{8}{c|}{\texttimes} \\
    & MSE & \multicolumn{8}{c|}{\texttimes} \\
    & SSIM & \multicolumn{8}{c|}{\texttimes} \\
    \hline
    \multirow{3}{*}{PNDM} & FID & \multicolumn{8}{c|}{\texttimes} \\
    & MSE & \multicolumn{8}{c|}{\texttimes} \\
    & SSIM & \multicolumn{8}{c|}{\texttimes} \\
    \hline
\end{tabular}
}
\caption{UIBDiff on VillanDiff of different samplers}
\label{tab:defense}
\end{table}
